Efficient Conditional Generation on Scale-based Visual Autoregressive Models

Recent advances in autoregressive (AR) models have demonstrated their potential to rival diffusion models in image synthesis. However, for complex spatially-conditioned generation, current AR approaches rely on fine-tuning the pre-trained model, leading to significant training costs. In this paper, we propose the Efficient Control Model (ECM), a plug-and-play framework featuring a lightweight control module that introduces control signals via a distributed architecture. This architecture consists of context-aware attention layers that refine conditional features using real-time generated tokens, and a shared gated feed-forward network (FFN) designed to maximize the utilization of its limited capacity and ensure coherent control feature learning. Furthermore, recognizing the critical role of early-stage generation in determining semantic structure, we introduce an early-centric sampling strategy that prioritizes learning early control sequences. This approach reduces computational cost by lowering the number of training tokens per iteration, while a complementary temperature scheduling during inference compensates for the resulting insufficient training of late-stage tokens. Extensive experiments on scale-based AR models validate that our method achieves high-fidelity and diverse control over image generation, surpassing existing baselines while significantly improving both training and inference efficiency.

==> tables/local_scalability.tex <==
\begin{table}[h]
    \centering
    \small
    \setlength{\tabcolsep}{1mm}
    \renewcommand{\arraystretch}{0.8}
    \caption{Analysis of scalability with different setup of adapter layers, sharing FFNs on VARd16 \cite{var}. FFN ratio represents the dimension of input and hidden states ratio of FFN.}
    \label{tab:local_scalability}
    \begin{tabular}{cccc|cc}
        \toprule
         \#Adapter & \#FFN & FFN Ratio & \#Param. & FID$\downarrow$ & IS$\uparrow$ \\
        \midrule
        3 & 1 & 4 & 52M & 5.80 & 179.07\\
        4 & 1 & 4 & 58M & 5.77 & \textbf{181.36}\\
        5 & 1 & 4 & 64M & \textbf{5.56} & 180.79\\
        4 & 2 & 4 & 69M & 5.85 & 180.90 \\
        4 & 1 & 6 & 62M & 5.82 & 179.02\\
        \bottomrule
    \end{tabular}
\end{table}
